Data-Driven Estimation of Heterogeneous Treatment Effects

Estimating how a treatment affects different individuals, known as heterogeneous treatment effect estimation, is an important problem in empirical sciences. In the last few years, there has been a considerable interest in adapting machine learning algorithms to the problem of estimating heterogeneous effects from observational and experimental data. However, these algorithms often make strong assumptions about the observed features in the data and ignore the structure of the underlying causal model, which can lead to biased estimation. At the same time, the underlying causal mechanism is rarely known in real-world datasets, making it hard to take it into consideration. In this work, we provide a survey of state-of-the-art data-driven methods for heterogeneous treatment effect estimation using machine learning, broadly categorizing them as methods that focus on counterfactual prediction and methods that directly estimate the causal effect. We also provide an overview of a third category of methods which rely on structural causal models and learn the model structure from data. Our empirical evaluation under various underlying structural model mechanisms shows the advantages and deficiencies of existing estimators and of the metrics for measuring their performance.

==> 00_abstract.tex <==
Estimating how a treatment affects different individuals, known as heterogeneous treatment effect estimation, is an important problem in empirical sciences. In the last few years, there has been a considerable interest in adapting machine learning algorithms to the problem of estimating heterogeneous effects from observational and experimental data. However, these algorithms often make strong assumptions about the observed features in the data and ignore the structure of the underlying causal model, which can lead to biased estimation. At the same time, the underlying causal mechanism is rarely known in real-world datasets, making it hard to take it into consideration. In this work, we provide a survey of state-of-the-art data-driven methods for heterogeneous treatment effect estimation, broadly categorizing them as methods that focus on counterfactual prediction and methods that directly estimate the causal effect. Our empirical evaluation under various underlying structural model mechanisms shows the advantages and deficiencies of existing estimators and of the metrics for measuring their performance. 


==> 03-03-scms.tex <==
\subsection{Data-driven HTE estimation using structure learning}\label{sec:structure_learning}

As mentioned in Section~\ref{sec:hte_estimation_with_scms}, when the structural causal model is known, an adjustment set can be used to select features for HTE estimation.
However, in many real-world scenarios, the underlying causal model is unknown, and therefore, there is \emph{structure uncertainty} of the causal mechanisms.
Therefore, ignoring the underlying causal models can lead to incorrect causal effect estimations.

To use the causal model under structure uncertainty, one approach is to use causal structure learning~\citep{heinze-stat18,vowels-arxiv21}.
Many traditional causal structure learning methods can be broadly classified into constraint-based~\citep{spirtes-book00,colombo-jstor12}, score-based~\citep{chickering-jmlr02,hauser-jmlr12,nandy-annals18}, a hybrid of the two~\citep{tsamardinos-ml06}, or based on asymmetries~\citep{shimizu-jmlr06}.
These methods find a partial graph or skeleton from the data, with some unoriented edges.
With the output from structure learning methods, an adjustment set can be applied to select variables for estimation~\citep{pearl-book09,henckel-arxiv19}, and these variables are used to train an HTE estimator.




Although causal structure learning can address some problems of data-driven HTE estimation, there are some drawbacks.
First, learning the full structure can be computationally expensive for high-dimensional datasets~\citep{chickering-jmlr04,heinze-stat18,vowels-arxiv21}.
Second, causal structure learning generally cannot learn the full causal model, so learned models will have undirected edges with an ambiguous cause-effect relationship.
In addition, adjustment criteria have been developed for total causal effect estimation without heterogeneity in mind.
Therefore, adjustment sets can potentially miss heterogeneity-inducing variables, leading to incorrect HTE estimation.
In our experiments, we use randomly generated SCMs and explore how data-driven HTE estimators perform under different types of SCMs.


==> __latexindent_temp.tex <==
\section{Heterogeneous Treatment Effects}\label{sec:background}

In this section, we provide background on heterogeneous treatment effect estimation, starting with notations from the perspective of the potential outcome framework~\citep{rubin1974}. Then we define the problem of heterogeneous treatment effect estimation and common assumptions to allow for estimation.
Finally, we introduce structural causal models~\citep{pearl-book09} and how they can be used to assess heterogeneity.

\subsection{Data model}\label{sec:data_model}

Before formalizing the problem and data model, we introduce the notations used in this survey. 
We denote a space of random variables with a calligraphic letter (e.g., $ \mathcal{X} $).
We denote random variables with a capital letter (e.g., $Y$) and random vectors with a boldfaced capital letter (e.g., $\mathbf{X}$).
Subscripts signify the random variable for a specific unit (e.g., $Y_i$ or $\mathbf{X}_i$).
Lowercase letters denote an assignment of a random variable or vector (e.g., $Y_i = y$ or $\mathbf{X}_i = \mathbf{x}$).
Each unit $i$ has a vector of ``pre-treatment'' features or covariates, $\mathbb{X}_i \in \mathcal{X}$, a binary treatment indicator, $T_i$, where $T_i=0$ and $T_i=1$ indicates $i$ is not treated and treated, respectively, and two outcomes when not treated and treated, $Y_i(T_i=0)$ and $Y_i(T_i=1)$, respectively.
The underlying data distribution is represented by a tuple $(\features_i, T_i, Y_i(0), Y_i(1))^N$ of $N$ independent and identically distributed individuals.
The average treatment effect (ATE) over the population is defined as the expected difference in potential outcomes:
\begin{equation}
    \label{eq:ate}
    \text{ATE} := E[Y(1) - Y(0)].
\end{equation}
The fundamental problem of causal inference is that for each individual, we can observe either the potential outcomes under treatment ($Y_i(1)$) or control ($Y_i(0)$), but not both. 
Therefore, we define the observed dataset as $\mathcal{D} = (\mathbf{x}_i, t_i, y_i)^N$ with $N$ individuals where $Y_i$ is defined as:
\begin{equation}
    \label{eq:potential_outcomes}
    Y_i = T_i Y_i(1) + (1 - T_i) Y_i(0).
\end{equation}
We denote $ Y_i $ as the factual outcome and the counterfactual outcome, $ Y_i' $, as the outcome that would have occurred if the treatment was different.

\subsection{Heterogeneous Treatment Effect Estimation}\label{sec:hte}

Since each unit reacts differently to treatment, we define the individual treatment effect (ITE) as the difference in the unit's potential outcomes, denoted by $\tau_i$:
\begin{equation}
    \label{eq:ite}
    \tau_i := Y_i(1) - Y_i(0).
\end{equation}
However, due to the fundamental problem of causal inference, $\tau_i$ is not observed for any individual.
The quantity of interest is often the conditional average treatment effect (CATE):
\begin{equation}
    \tau(\mathbf{x}) := \mathbb{E} \left[ Y_i(1) - Y_i(0) \mid \features_i = \mathbf{x} \right].
\end{equation}
The CATE describes the expected treatment effect for units in a subpopulation with features $\mathbf{x}$.
The best estimator for CATE is also the best estimator for ITE in terms of the mean squared error~\citep{kunzel-pnas19}, though in general, the ITE is not the same as CATE~\citep{vegetabile-arxiv21}.
The goal of HTE estimation is to develop estimators of CATE which have the smallest root mean squared error for the ITE.
\begin{problem}\label{prob:hte_problem}
    (Heterogeneous treatment effect estimation)
    Given a dataset $\mathcal{D}=(\features_i, Y_i, T_i)$ of N instances with some true ITE. $\tau_i$, estimate CATE $\hat{\tau}(\mathbf{X})$ such that the root mean squared error (RMSE) is minimized:
    \begin{equation}\label{eq:cate_objective}
         \minl_{\hat{\tau}} \text{RMSE} = \frac{1}{N} \sum_{i=1}^N  (\tau_i - \hat{\tau}(\mathbf{X}_i)) ^ 2.
    \end{equation}
\end{problem}

\subsection{HTE Assumptions}\label{sec:hte_assumptions}

In order to estimate HTEs from observational data, some assumptions on the set of features and data given are needed.
We present some common assumptions used in heterogeneous treatment effect estimators.

\begin{assumption}\label{assumption:strong_ignorability}
    (Strong Ignorability) Given a binary treatment $T$, potential outcomes $Y(0)$, $Y(1)$, and a vector of features or covariates $\features$, strong ignorability states:
    \begin{align}
        \{ Y(0), Y(1) \} \perp T \mid \features,
    \end{align}
\end{assumption}
This states the \emph{potential} outcomes are conditionally independent of the treatment conditioned on the features.
When strong ignorability holds, $\features$ is said to be ``admissible'', meaning treatment effects can be estimated without bias.
This assumption is also known as unconfoundedness or the assumption of no hidden confounding.

\begin{assumption}\label{assumption:overlap}
    (Population Overlap) $0 < P(T_i = 1) < 1$ with probability 1.
\end{assumption}
This assumption states that all units have a non-zero probability of assignment to each treatment condition.
Assumption~\ref{assumption:overlap} is also known as positivity or common support.

Another common assumption used is the Stable Unit Treatment Value Assumption (SUTVA) or the assumption of no interference~\citep{rubin-jasa80}.
\begin{assumption}\label{assumption:sutva}
    (Stable Unit Treatment Value Assumption (SUTVA)) Given two individuals $i, j$, the potential outcomes of $i$, $\{Y_i(0), Y_i(1) \}$ are unaffected by the treatment assignment of other individuals $\forall j$:
    \begin{equation}
        \{Y_i(0), Y_i(1)\} \perp T_j, \forall j \neq i.
    \end{equation}
    SUTVA is also often referred to as the assumption of ``no interference''.
\end{assumption}
With the SUTVA assumption, individual outcomes are not affected by treatment or outcomes of peers.
Though there has been some work focused on estimating HTEs without the SUTVA assumption~\citep{yuan-www21,tran-aaai22}, a majority of work in HTE estimation has focused on non-networked settings, which we focus on in this survey.

\subsection{Data-driven HTE Estimation}\label{sec:data_driven_background}

Given an observed dataset $\mathcal{D}$, the goal of an \emph{HTE estimator} is to estimate CATE, $\hat{\tau}$, using the available features $\features$ in the data.
HTE estimators estimate CATE in a variety of ways.
Some HTE estimators rely on recursive partitioning using tree-based methods~\citep{tran-aaai19,athey-pnas16,athey-annals19}.
Other HTE estimators use predictions from machine learning methods to train a causal effect estimator~\citep{kunzel-pnas19,kennedy-arxiv20} or to predict counterfactual outcomes for estimation of effect~\citep{shalit-icml17,johansson-icml16}.
We describe these methods in Section~\ref{sec:survey}.

Since the true ITE is unknown in real-world scenarios, several heuristic HTE evaluation metrics have been developed for evaluating the performance of HTE estimators.
These metrics include inverse propensity weighting (IPW) validation~\citep{schuler-model18}, $ \tau $-risk~\citep{schuler-model18,nie-rlearner17}, nearest-neighbor imputation (NN-PEHE)~\citep{schwab-perfect18}, plugin validation~\citep{saito-cv19}, and counterfactual cross-validation (CFCV)~\citep{saito-cv19}. 

IPW validation uses inverse propensity score weighting to a plugin estimate for the CATE, $ \tilde{\tau} $~\citep{schuler-model18}:
\begin{equation}
    \tilde{\tau}_{IPW} (\mathbf{X}_i, Y_i, T_i) = \frac{T_i}{\hat{e}(\mathbf{X}_i)}Y_i - \frac{1 - T_i}{1 - \hat{e}(\mathbf{X}_i)} Y_i.
\end{equation}
Here, $ \hat{e}(\mathbf{x}) $ is an estimate of the propensity score (i.e., $\mathbb{E}[T_i|\mathbf{X}_i]$)
This plugin is used to approximate the mean-squared error for the estimator $ \hat{\tau} $:
\begin{equation}
    \hat{R}_{IPW}(\hat{\tau}) = \frac{1}{n} \sum_{i=1}^n \Big(\tilde{\tau}_{IPW} (\mathbf{X}_i, Y_i, T_i) - \hat{\tau}(\mathbf{X}_i) \Big)^2.
\end{equation}

The $ \tau  $-risk takes as input an estimator $ \hat{\tau}  $ and approximates the objective defined in~\eqref{eq:cate_objective}.
To do this, two functions are defined: $ \hat{m}(\mathbf{X}_i) $ which is an outcome estimator for unit $i$ (i.e., $ \mathbb{E}[Y_i | \mathbf{X}_i] $) and $ \hat{e}(\mathbf{X}_i) $ which is an estimate of the propensity score.
Both $ \hat{m} $ and $ \hat{e} $ are learned through supervised techniques and optimized for predictive accuracy~\citep{nie-rlearner17}.
The $ \tau  $-risk is defined as:
\begin{equation}
    \tau\text{-risk} = \frac{1}{N} \sum_{i=1}^N \Big( \big(Y_i-\hat{m}(\mathbf{X}_i)\big) - \big(T_i - \hat{e}(\mathbf{X}_i)\big)\hat{\tau}(\mathbf{X}_i) \Big)^2.
\end{equation}

Nearest neighbor precision in estimation of heterogeneous effects (NN-PEHE) uses matching to approximate a treatment effect by substituting counterfactual outcomes from matched neighbors~\citep{schwab-perfect18}.
A unit $i$ is matched with one\footnote{Matching can be done with multiple units, and an aggregate can be computed.} control and one treated unit, denoted by NN$_0 (i)$ and NN$_1 (i)$. 
Using the matched units, a substitute of the ground-truth treatment effect is computed as $ y(\text{NN}_1(i)) - y(\text{NN}_0(i)) $.
The NN-PEHE error, $ \hat{\epsilon}_{\text{NN-PEHE}} $ is computed as:
\begin{equation}
    \hat{\epsilon}_{\text{NN-PEHE}} = \frac{1}{N} \sum_{i=1}^n \bigg( \big(y(\text{NN}_1(i)) - y(\text{NN}_0(i)) \big) - \hat{\tau}(\mathbf{X}_i) \bigg)^2.
\end{equation}

Plugin validation uses arbitrary machine learning algorithms to estimate a plugin $ \tau $, similar to IPW validation.
To get a plugin estimate, two predictions are needed, $ f_1(\mathbf{x}) $ and $ f_0(\mathbf{{x}}) $, which are predictions of the outcome when treated and not treated, respectively, using only the features.
Then, the plugin validation metric is defined as:
\begin{equation}
    \hat{R}_{plugin}(\hat{\tau}) = \frac{1}{N} \sum_{i=1}^N \bigg( (f_1(\mathbf{X}_i) - f_0(\mathbf{X}_i)) - \hat{\tau}(\mathbf{X}_i) \bigg)^2.
\end{equation}

Counterfactual cross-validation (CFCV) uses the plugin estimate of the CATE in a doubly robust formulation~\citep{saito-cv19}:
\begin{equation}
    \tilde{\tau}_{DR}(\mathbf{X}_i, Y_i, T_i) = \frac{T - \hat{e}(\mathbf{X}_i)}{\hat{e}(\mathbf{X}_i) (1 - \hat{e}(\mathbf{X}_i))} (Y_i - f_T(\mathbf{X}_i)) + f_1(\mathbf{X}_i) - f_0(\mathbf{X}_i),
\end{equation}
where $ \hat{e} $ is an estimate of the propensity score and $ f_t(\mathbf{x}) $ is an arbitrary regression function for a specific treatment value $ t $ that predicts the outcome given the set of features.
Then, the plugin estimate $ \tilde{\tau}_{DR} $ can be used in the mean-squared error estimate:
\begin{equation}
    \hat{R}_{CFCV} = \frac{1}{N} \sum_{i=1}^N \bigg( \tilde{\tau}_{DR}(\mathbf{X}_i, Y_i, T_i) - \hat{\tau}(\mathbf{X}_i) \bigg)^2
\end{equation}

Each metric is an estimate of the error of an HTE estimator and performance based on these heuristic metrics has been shown to correlate with true performance.
Since these metrics are heuristic, we explore their reliability in synthetic and semi-synthetic experiments in Section~\ref{sec:experiments}.

\subsection{Structural Causal Models}\label{sec:scm_background}

\begin{figure}
    \centering
    \newcommand{\scmsize}{0.5}
        \begin{subfigure}[b]{\columnwidth}
            \centering
            \begin{tikzpicture}
                \node (t) at (-0.75, 0) [label=below:$T$,point];
                \node (x) at (0.0, 0.75) [label=left:\(X\),point];
                \node(y) at (0.75, 0.0) [label=below:$Y$,point];
                \node (ux) at (0.0, 1.5) [label=above:\(U_X\),point];
                \node (ut) at (-1.5, 0.75) [label=above:\(U_T\),point];
                \node (uy) at (1.5, 0.75) [label=above:\(U_Y\),point];

                \path (x) edge (t);
                \path (x) edge (y);
                \path (t) edge (y);
                \path (ux) edge (x);
                \path (uy) edge (y);
                \path (ut) edge (t);
            \end{tikzpicture}
        \end{subfigure}
    \caption{An example causal model.
    }\label{fig:example_scm}
\end{figure}

Now we introduce an alternative to data-driven estimation of causal effects through structural causal models (SCMs) and how they relate to heterogeneous effects.

A structural causal model (SCM), $M$, consists of two sets of variables, $\mathbf{U}$ and $\mathbf{V}$, and a set of structural equations, $\mathbf{F}$, describing how values are assigned to each \emph{endogenous} variable $V^{(i)} \in \mathbf{V}$ based on the values of $\mathbf{v}$ and $\mathbf{u}$~\citep{pearl-book09}: \( v^{(i)} = f^{(i)}(\mathbf{v}, \mathbf{u}) \).
A causal graph \( G \) is a directed acyclic graph that captures the causal relationships among the variables.
Each variable, $V^{(i)}$, is represented by a node in the causal graph, an edge from $V^{(i)}$ to $V^{(j)}$ signifies that $V^{(i)}$ is a cause of $V^{(j)}$.
We also refer to the edge relationship as a parent-child relationship, where the parent is a cause of the child.
The variables in $\mathbf{U}$ are considered \emph{exogenous}, and the causal graph may omit representing $\mathbf{U}$ explicitly.
Figure~\ref{fig:example_scm} shows an example of a causal graph with three exogenous variables, $ U_X, U_T, U_Y $ and three endogenous variables, $ X, T, Y $. 
An example set of associated structural equations is shown in eq~\eqref{eq:see1}-\eqref{eq:see3}.
\begin{gather}
    X = U_X \label{eq:see1} \\
    T = Bern(X) + U_T \label{eq:see2}  \\
    Y = \alpha \cdot T + \beta \cdot X + U_Y \label{eq:see3} 
\end{gather}
Here, each endogenous variable has a directed edge pointing to it from an exogenous variable (e.g., $ U_X \rightarrow X $ or $ U_T $ is a parent of $ X $).
This is represented in the structural equations as being part of the structural equation (e.g., $ U_X $ in eq~\eqref{eq:see1}).
It is assumed that every endogenous variable has a parent in $ \mathbf{U} $.
We denote the parents and children of a variable, $ X $, in the graph as $ pa(X) $ and $ ch(X) $, respectively.
Ancestors of $ X $, $ an(X) $, are variables that can reach $ X $ through a directed path, and descendants of $ X $, $ de(X) $, are variables that can be reached from $ X $ through directed paths out of $ X $.

\subsubsection{Identifying effects using SCMs}\label{sec:identifying_scms}

When the SCM underlying the dataset is known, its graph $ G $ supports the use of graphical criteria for variable selection for unbiased causal effect estimation, known as adjustment set selection~\citep{shpitser-uai06,shpitser-uai10,van-uai14,perkovic-uai15,henckel-arxiv19}.
These graphical criteria rely on the concept of $d$-separation.
\begin{definition}
    ($d$-separation) A set of $ \mathbf{Z} $ nodes is said to ``block'' a path $ p $ if either
    \begin{enumerate}
        \item[$(i)$] $ p $ contains at least one arrow-emitting node that is in $ \mathbf{Z} $ or
        \item[$(ii)$] $p$ contains at least one collision node that is outside $ \mathbf{Z} $ and has no descendant in $ \mathbf{Z} $.
    \end{enumerate}
\end{definition}
If $ \mathbf{Z} $ blocks all paths from a set of nodes $ \mathbf{X} $ to a set of nodes $ \mathbf{Y} $, it is said to ``d-separate'' $ \mathbf{X} $ and $ \mathbf{Y} $, and the conditional independence, $ \mathbf{X} \perp \mathbf{Y} \mid \mathbf{Z} $, holds~\citep{bareinboim-pnas16}.
One graphical criteria for adjustment set selection is the backdoor criterion~\citep{pearl-book09}.
The backdoor criterion aims to find a set that \emph{blocks} the paths from the treatment variable to the outcome variable in the graph, starting with an arrow into the treatment variable.
Essentially, the backdoor criterion blocks all the paths going backwards out of treatment.
For example, in Figure~\ref{fig:example_scm}, there is one backdoor path, namely $ T \leftarrow X \rightarrow Y $, and so the adjustment set $ \{X\} $ sufficiently satisfies the backdoor criterion.
Several adjustment criteria have been developed, such as the adjustment criterion~\citep{shpitser-uai06,van-uai14}, generalized backdoor criterion~\citep{maathuis-annals15}, generalized adjustment criterion~\citep{perkovic-uai15}, and optimal adjustment set (O-set)~\citep{henckel-arxiv19}.
These adjustment sets defined by the various adjustment criteria can be found through \emph{identification} algorithms such as the ID algorithm~\citep{shpitser-jmlr08}, the algorithmic framework by Van der Zander et al.~\citep{van-uai14} or the pruning procedure by Henckel et al.~\citep{henckel-arxiv19}.

When an adjustment set is discovered, unbiased causal effects can be estimated by conditioning on the adjustment set. 
The adjustment set can be used instead of all the features for data-driven estimation.
We discuss data-driven HTE estimation with SCMs briefly in Section~\ref{sec:hte_estimation_with_scms}.

\subsubsection{C-specific effects}

Shpitser and Pearl provide a nonparametric estimand for HTEs for some feature assignment $C=c$, called $c$-specific effects~\citep{shpitser-uai06,pearl-smr17}.
One issue with estimating $c$-specific effects is that it requires knowledge of the SCM and which variables, C, exhibit heterogeneous effects.
When the SCM is known, the O-set~\citep{henckel-arxiv19} can be used on the learned structure since it implicitly includes all potential heterogeneity-inducing variables, while some identification algorithms may miss them. When the SCM is unknown, the identifiability of \( c \)-specific effects cannot be established. 
Moreover, when the set of heterogeneity-inducing variables $\mathbf{C}$ is unknown, then all combinations of features and feature values would need to be checked for heterogeneity in effect, which is exponential in the number of valid features. 
Circumventing this exponential search is one of the main reasons data-driven methods are popular in practice.

Shpitser and Pearl provide a nonparametric estimand for HTEs with respect to some feature assignment $C=c$, called $c$-specific effects~\citep{shpitser-uai06,pearl-smr17}.
There are three cases when $c$-specific effects are \emph{identifiable}, i.e., there exists an unbiased estimation for $\tau(\mathbf{c}) = E[Y(1) - Y(0) | \mathbf{C}=\mathbf{c}]$.
The first case is when $\mathbf{C}$ is observed and admissible which means that it satisfies the backdoor criterion in the causal graph~\citep{pearl-book09}.
A set of variables $\mathbf{Z}$ satisfies the backdoor criterion relative to $(T,Y)$ if no node in $\mathbf{Z}$ is a descendant of $T$ and $\mathbf{Z}$ blocks every path between $T$ and $Y$ that contains an arrow into $T$.
For example, $X$ is the only variable that is admissible in all SCMs in Figure~\ref{fig:fail_examples}, since it blocks the only backdoor path.

The second case is when $\mathbf{C}$ is part of an observed admissible set.
In this case, $\mathbf{C}$ itself is not admissible, but we can observe a set of features $\mathbf{S}$ such that $\mathbf{S} \cup \mathbf{C}$ is admissible.
In Figure~\ref{fig:marloes_scm}, $\{F\}$ could induce heterogeneity but is not admissible on its own. Adding $F$ to $\{X\}$ still satisfies the backdoor criterion making $\{X, F\}$ also admissible.
The third case for identifiable $c$-specific effects is when $\mathbf{C}$ is not part of an admissible set.
The first two cases which rely on \emph{covariate adjustment}~\citep{perkovic-jmlr18} and identifying heterogeneity-inducing variables are the basis of our work.
Estimating heterogeneous effects in the third case is beyond the scope of this paper and is reserved for future work. 

One issue with estimating $c$-specific effects is that it requires knowledge of the SCM and which variables exhibit heterogeneous effects.
If the SCM is unknown, the identifiability of \( c \)-specific effects cannot be established.
If $\mathbf{C}$ is unknown, then all combinations of features and feature values would need to be checked for heterogeneity in effect, which is exponential in the number of valid features.
Circumventing this exponential search is one of the main reasons why data-driven methods are popular in practice.

\subsubsection*{Detecting latent heterogeneity}

In some cases, the observed covariates that induce heterogeneity, $C$, are not known, but there is unknown heterogeneity in effects present in the data~\citep{pearl-smr17}.
Pearl discusses how heterogeneity can be detected from statistical averages alone~\citep{pearl-smr17} when the effect of treatment on the treated (ETT) and the effect of treatment on the untreated (ETU) are identifiable.

\subsubsection{HTEs in SCMs}\label{sec:htes_scms_background}

In SCMs, heterogeneous effects are represented by an \emph{interaction} or \emph{effect modification} through ancestors and parents of a variable.
In a linear structural equation, an interaction occurs as a multiplication of two variables.
For heterogeneous effects, this interaction is specifically with the treatment variable.
Consider the causal model in Figure~\ref{fig:example_scm}, where the treatment variable of interest is $ T $ and the outcome of interest is $ Y $.
There is a potential interaction between $ X $ and $ T $.
Suppose $ Y $ is generated by the following structural equation:
\begin{equation}
    Y = \alpha \cdot T + \beta \cdot X + \gamma \cdot T \cdot X + U_Y.
\end{equation}
Here, there is a fixed effect \( \alpha \) of the treatment \( T \) and a heterogeneous effect \( \gamma \) due to the interaction between \( T \) and \( X \).
Since the effect of treatment varies with another variable, $ X $, there is a heterogeneous effect.
Heterogeneity through interaction can occur with any parent of the outcome or any parent of \emph{mediating} variables~\citep{vanderweele-epid07}.
Consider another example causal model, shown in Figure~\ref{fig:multi_interaction}.
Here, there is a \emph{mediating} variable, $ D $, a variable that occurs on a path from the treatment, $ T $, to the outcome, $ Y $.
Interaction can occur with $ X, C$, or $ F $.
For example, an interaction with $ X $ and $ F $ can be shown as:
\begin{equation}
    Y = \alpha \cdot D \cdot X + \beta \cdot D \cdot F + U_Y.
\end{equation}
Since the treatment is mediated through $ D $ and $ X $ and $ F $ interact with $ D $, there will be a heterogeneous effect.
Since $ D $ is a mediator, if $ C $ interacts with $ T $ in the structural equation, then there will also be a heterogeneous effect, such as:
\begin{gather}
    D = \alpha \cdot T + \beta \cdot T \cdot C + U_D, \\
    Y = \gamma \cdot D + U_Y.
\end{gather}

\begin{figure}
    \centering
    \begin{tikzpicture}
        \node (t) at (-1.5, 0) [label={below left}:$T$,point];
        \node (x) at (-1.5, 1.5) [label={above}:$X$,point];
        
        \node (c) at (0.0, 1.5) [label={above}:$C$,point];
        \node (d) at (0.0, 0) [label={below}:$D$,point];

        \node (f) at (1.5, 1.5) [label={above}:$F$,point];
        \node (y) at (1.5, 0.0) [label={below}:$Y$,point];

        \path (x) edge (t);
        
        \path (x) edge (y);
        \path(t)edge(d);
        \path(c)edge(d);
        \path (d) edge (y);

        \path (f) edge (y);
    \end{tikzpicture}
    \caption{Causal model with multiple possible interactions that cause heterogeneous treatment effects.}\label{fig:multi_interaction}
\end{figure}




                
        
        
                
        




